Design Space Exploration as Quantified Satisfaction

We present novel algorithms for design and design space exploration. The designs discovered by these algorithms are compositions of function types specified in component libraries. Our algorithms reduce the design problem to quantified satisfiability and use advanced solvers to find solutions that represent useful systems. The algorithms we present in this paper are sound and complete and are guaranteed to discover correct designs of optimal size, if they exist. We apply our method to the design of Boolean systems and discover new and more optimal classical digital and quantum circuits for common arithmetic functions such as addition and multiplication. The performance of our algorithms is evaluated through extensive experimentation. We created a benchmark consisting of specifications of scalable synthetic digital circuits and real-world mirochips. We have generated multiple circuits functionally equivalent to the ones in the benchmark. The quantified satisfiability method shows more than four orders of magnitude speed-up, compared to a generate and test method that enumerates all non-isomorphic circuit topologies. Our approach generalizes circuit optimization. It uses arbitrary component libraries and has applications to areas such as digital circuit design, diagnostics, abductive reasoning, test vector generation, and combinatorial optimization.

==> figures/pgflibrarycolors.code.tex <==
\definecolor{antiquewhite}{rgb}{0.98, 0.92, 0.84}
\definecolor{champagne}{rgb}{0.97, 0.91, 0.81}
\definecolor{darkkhaki}{rgb}{0.74, 0.72, 0.42}
\definecolor{pastelgray}{rgb}{0.81, 0.81, 0.77}
\definecolor{whitesmoke}{rgb}{0.96, 0.96, 0.96}
\definecolor{tearose(rose)}{rgb}{0.96, 0.76, 0.76}


==> figures/pgflibrarydots.code.tex <==
\newcommand{\smallVerticalDots}[1]{
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 + (0, 0.1)$) {};
  \node[fill=black, circle, inner sep=0.25pt] at #1 {};
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 - (0, 0.1)$) {};
}

\newcommand{\smallDiagonalDots}[1]{
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 + (-0.1, 0.1)$) {};
  \node[fill=black, circle, inner sep=0.25pt] at #1 {};
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 + (0.1, -0.1)$) {};
}

\newcommand{\mediumDiagonalDots}[1]{
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (-0.125, 0.125)$) {};
  \node[fill=black, circle, inner sep=0.5pt] at #1 {};
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (0.125, -0.125)$) {};
}

\newcommand{\smallHorizontalDots}[1]{
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 + (-0.1, 0)$) {};
  \node[fill=black, circle, inner sep=0.25pt] at #1 {};
  \node[fill=black, circle, inner sep=0.25pt] at ($#1 + (0.1, 0)$) {};
}

\newcommand{\mediumHorizontalDots}[1]{
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (-0.15, 0)$) {};
  \node[fill=black, circle, inner sep=0.5pt] at #1 {};
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (0.15, 0)$) {};
}

\newcommand{\mediumVerticalDots}[1]{
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (0, -0.15)$) {};
  \node[fill=black, circle, inner sep=0.5pt] at #1 {};
  \node[fill=black, circle, inner sep=0.5pt] at ($#1 + (0, 0.15)$) {};
}


==> figures/pgflibraryn_adder.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\pgfdeclareshape{rc adder}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=1.75\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-1.75\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
 \anchor{in 1}{
   \northwest
   \pgf@x=-0.4\pgf@x
   \pgf@y=\pgf@y
 }
 \anchor{in 2}{
   \northwest
   \pgf@x=0.4\pgf@x
   \pgf@y=\pgf@y
 }
 \anchor{out}{
   \northwest
   \pgf@x=0pt
   \pgf@y=-\pgf@y
 }
 \anchor{in c}{
   \northwest
   \pgf@x=-\pgf@x
   \pgf@y=0pt
 }
 \anchor{out c}{
   \northwest
   \pgf@x=\pgf@x
   \pgf@y=0pt
 }

  \backgroundpath{

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y 
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgfscope

    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@up}} % i1
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{\pgf@circ@res@up}} % i2
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}} % out
    \pgfpathlineto{\pgfpoint{0}{0.5\pgf@circ@res@down}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}} % cin
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}} % cout
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@left}{0}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfsetlinewidth{2\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfclosepath
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope
  }
}
\makeatother


==> figures/pgflibraryn_multi_operand_adder.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\newdimen\pgf@ca@up
\newdimen\pgf@ca@down
\newdimen\pgf@ca@left
\newdimen\pgf@ca@right

\pgf@ca@up=.35cm
\pgf@ca@down=-.35cm
\pgf@ca@left=-.4cm
\pgf@ca@right=.4cm

\pgfdeclareshape{ca}{
  \nodeparts{text}

  \anchor{center}{\pgfpointorigin}
  \anchor{a 1}{\pgfpoint{0}{\pgf@ca@up}}
  \anchor{o 1}{\pgfpoint{0}{\pgf@ca@down}}
  \anchor{ci}{\pgfpoint{\pgf@ca@left}{0}}
  \anchor{co}{\pgfpoint{\pgf@ca@right}{0}}
  \anchor{text}{
    \pgf@x=-.5\wd\pgfnodeparttextbox
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@ca@left}{\pgf@ca@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ca@right}{\pgf@ca@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ca@right}{\pgf@ca@down}}
    \pgfpathlineto{\pgfpoint{\pgf@ca@left}{\pgf@ca@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope

    \pgfpathmoveto{\pgfpoint{0}{0}}
  }
}

\newdimen\pgf@cb@up
\newdimen\pgf@cb@down
\newdimen\pgf@cb@left
\newdimen\pgf@cb@right

\pgf@cb@up=.35cm
\pgf@cb@down=-.35cm
\pgf@cb@left=-.525cm
\pgf@cb@right=.525cm

\pgfdeclareshape{cb}{
  \nodeparts{text}

  \anchor{center}{\pgfpointorigin}
  \anchor{a 1}{\pgfpoint{0.5\pgf@cb@left}{\pgf@cb@up}}
  \anchor{a 2}{\pgfpoint{0.5\pgf@cb@right}{\pgf@cb@up}}
  \anchor{o 1}{\pgfpoint{0.5\pgf@cb@left}{\pgf@cb@down}}
  \anchor{o 2}{\pgfpoint{0.5\pgf@cb@right}{\pgf@cb@down}}
  \anchor{ci}{\pgfpoint{\pgf@cb@left}{0}}
  \anchor{co}{\pgfpoint{\pgf@cb@right}{0}}
  \anchor{text}{
    \pgf@x=-.5\wd\pgfnodeparttextbox
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@cb@left}{\pgf@cb@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cb@right}{\pgf@cb@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cb@right}{\pgf@cb@down}}
    \pgfpathlineto{\pgfpoint{\pgf@cb@left}{\pgf@cb@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope
  }
}

\newdimen\pgf@cc@up
\newdimen\pgf@cc@down
\newdimen\pgf@cc@left
\newdimen\pgf@cc@right

\pgf@cc@up=.35cm
\pgf@cc@down=-.35cm
\pgf@cc@left=-.7cm
\pgf@cc@right=.7cm

\pgfdeclareshape{cc}{
  \nodeparts{text}

  \anchor{center}{\pgfpointorigin}
  \anchor{a 1}{\pgfpoint{0.625\pgf@cc@left}{\pgf@cc@up}}
  \anchor{a 2}{\pgfpoint{0}{\pgf@cc@up}}
  \anchor{a 3}{\pgfpoint{0.625\pgf@cc@right}{\pgf@cc@up}}
  \anchor{o 1}{\pgfpoint{0.625\pgf@cc@left}{\pgf@cc@down}}
  \anchor{o 2}{\pgfpoint{0}{\pgf@cc@down}}
  \anchor{o 3}{\pgfpoint{0.625\pgf@cc@right}{\pgf@cc@down}}
  \anchor{ci}{\pgfpoint{\pgf@cc@left}{0}}
  \anchor{co}{\pgfpoint{\pgf@cc@right}{0}}
  \anchor{text}{
    \pgf@x=-.5\wd\pgfnodeparttextbox
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@cc@left}{\pgf@cc@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cc@right}{\pgf@cc@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cc@right}{\pgf@cc@down}}
    \pgfpathlineto{\pgfpoint{\pgf@cc@left}{\pgf@cc@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope
  }
}

\newdimen\pgf@cd@up
\newdimen\pgf@cd@down
\newdimen\pgf@cd@left
\newdimen\pgf@cd@right

\pgf@cd@up=.35cm
\pgf@cd@down=-.35cm
\pgf@cd@left=-.875cm
\pgf@cd@right=.875cm

\pgfdeclareshape{cd}{
  \nodeparts{text}

  \anchor{center}{\pgfpointorigin}

  \anchor{a 1}{\pgfpoint{0.75\pgf@cd@left}{\pgf@cd@up}}
  \anchor{a 2}{\pgfpoint{0.25\pgf@cd@left}{\pgf@cd@up}}
  \anchor{a n}{\pgfpoint{0.75\pgf@cd@right}{\pgf@cd@up}}

  \anchor{o 1}{\pgfpoint{0.75\pgf@cd@left}{\pgf@cd@down}}
  \anchor{o 2}{\pgfpoint{0.25\pgf@cd@left}{\pgf@cd@down}}
  \anchor{o n}{\pgfpoint{0.75\pgf@cd@right}{\pgf@cd@down}}

  \anchor{ci}{\pgfpoint{\pgf@cd@left}{0}}
  \anchor{co}{\pgfpoint{\pgf@cd@right}{0}}

  \anchor{text}{
    \pgf@x=-.5\wd\pgfnodeparttextbox
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@cd@left}{\pgf@cd@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cd@right}{\pgf@cd@up}}
    \pgfpathlineto{\pgfpoint{\pgf@cd@right}{\pgf@cd@down}}
    \pgfpathlineto{\pgfpoint{\pgf@cd@left}{\pgf@cd@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope
  }
}

\makeatother


==> figures/pgflibraryn_shifter.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\pgfdeclareshape{mux two}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=1.75\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-1.75\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \anchor{in 1}{
    \northwest
    \pgf@x=\pgf@x
    \pgf@y=0.4\pgf@y
  }
  \anchor{in 2}{
    \northwest
    \pgf@x=\pgf@x
    \pgf@y=-0.4\pgf@y
  }
  \anchor{out}{
    \northwest
    \pgf@x=-\pgf@x
    \pgf@y=0.4\pgf@y
  }
  \anchor{sel in}{
    \northwest
    \pgf@x=0pt
    \pgf@y=-\pgf@y
  }
  \anchor{sel out}{
    \northwest
    \pgf@x=0pt
    \pgf@y=\pgf@y
  }

  \backgroundpath{

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y 
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgfscope

    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@left}{0.4\pgf@circ@res@up}} % i1
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@left}{0.4\pgf@circ@res@down}} % i2
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.4\pgf@circ@res@up}} % out
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@up}} % sout
    \pgfpathlineto{\pgfpoint{0}{0.75\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}} % sin
    \pgfpathlineto{\pgfpoint{0}{0.75\pgf@circ@res@down}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfsetlinewidth{2\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfclosepath
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope
  }
}
\makeatother


==> figures/pgflibraryn_subtractor.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\pgfdeclareshape{rc subtractor}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=1.75\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-1.75\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
 \anchor{in 1}{
   \northwest
   \pgf@x=-0.4\pgf@x
   \pgf@y=\pgf@y
 }
 \anchor{in 2}{
   \northwest
   \pgf@x=0.4\pgf@x
   \pgf@y=\pgf@y
 }
 \anchor{out}{
   \northwest
   \pgf@x=0pt
   \pgf@y=-\pgf@y
 }
 \anchor{in b}{
   \northwest
   \pgf@x=-\pgf@x
   \pgf@y=0pt
 }
 \anchor{out b}{
   \northwest
   \pgf@x=\pgf@x
   \pgf@y=0pt
 }

  \backgroundpath{

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y 
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgfscope

    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@up}} % i1
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{\pgf@circ@res@up}} % i2
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}} % out
    \pgfpathlineto{\pgfpoint{0}{0.5\pgf@circ@res@down}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}} % cin
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}} % cout
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@left}{0}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw}

    \pgfsetlinewidth{2\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfclosepath
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope
  }
}
\makeatother


==> figures/pgflibraryref.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}
\pgfkeys{/tikz/refsize/.initial=1cm}

\newdimen\pgf@ref@up
\newdimen\pgf@ref@down
\newdimen\pgf@ref@left
\newdimen\pgf@ref@right

\pgf@ref@up=.15cm
\pgf@ref@down=-.15cm
\pgf@ref@left=0cm

\pgfdeclareshape{ref}{
  \nodeparts{text}

  \saveddimen{\pgf@ref@right}{\pgf@x=\pgfkeysvalueof{/tikz/refsize}}

  \anchor{center}{\pgfpointorigin}
  \anchor{west}{\pgfpoint{\pgf@ref@left}{0}}

  \anchor{in}{\pgfpoint{\pgf@ref@left}{0}}
  \anchor{out}{\pgfpoint{\pgf@ref@right}{0}}

  \anchor{text}{
    \pgf@x=1.5pt
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@ref@left}{\pgf@ref@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right-0.225cm}{\pgf@ref@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right-0.225cm}{\pgf@ref@down}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@left}{\pgf@ref@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope
  }
}

\makeatother


==> figures/pgflibrarystd_gates.code.tex <==
\makeatletter

\ctikzset{tripoles/and gate/width/.initial=1.1}
\ctikzset{tripoles/and gate/height/.initial=.8}
\ctikzset{tripoles/and gate/port width/.initial=.7}
\ctikzset{tripoles/and gate/input height/.initial=.5}
\ctikzset{tripoles/nand gate/width/.initial=1.1}
\ctikzset{tripoles/nand gate/height/.initial=.8}
\ctikzset{tripoles/nand gate/port width/.initial=.7}
\ctikzset{tripoles/nand gate/circle width/.initial=.15}
\ctikzset{tripoles/nand gate/input height/.initial=.5}
\ctikzset{tripoles/or gate/width/.initial=1.1}
\ctikzset{tripoles/or gate/height/.initial=.8}
\ctikzset{tripoles/or gate/port width/.initial=.7}
\ctikzset{tripoles/or gate/input height/.initial=.5}
\ctikzset{tripoles/or gate/input skip/.initial=.25}
\ctikzset{tripoles/or gate/aaa/.initial=.6}
\ctikzset{tripoles/or gate/bbb/.initial=.4}
\ctikzset{tripoles/or gate/ccc/.initial=.5}
\ctikzset{tripoles/or gate/ddd/.initial=.0}
\ctikzset{tripoles/nor gate/width/.initial=1.1}
\ctikzset{tripoles/nor gate/height/.initial=.8}
\ctikzset{tripoles/nor gate/port width/.initial=.7}
\ctikzset{tripoles/nor gate/input height/.initial=.5}
\ctikzset{tripoles/nor gate/input skip/.initial=.25}
\ctikzset{tripoles/nor gate/circle width/.initial=.15}
\ctikzset{tripoles/nor gate/aaa/.initial=.6}
\ctikzset{tripoles/nor gate/bbb/.initial=.4}
\ctikzset{tripoles/nor gate/ccc/.initial=.5}
\ctikzset{tripoles/nor gate/ddd/.initial=.0}
\ctikzset{tripoles/xor gate/width/.initial=1.1}
\ctikzset{tripoles/xor gate/height/.initial=.8}
\ctikzset{tripoles/xor gate/port width/.initial=.7}
\ctikzset{tripoles/xor gate/input height/.initial=.5}
\ctikzset{tripoles/xor gate/input skip/.initial=.15}
\ctikzset{tripoles/xor gate/distance/.initial=.1}
\ctikzset{tripoles/xor gate/aaa/.initial=.6}
\ctikzset{tripoles/xor gate/bbb/.initial=.4}
\ctikzset{tripoles/xor gate/ccc/.initial=.5}
\ctikzset{tripoles/xor gate/ddd/.initial=.0}
\ctikzset{tripoles/xnor gate/width/.initial=1.1}
\ctikzset{tripoles/xnor gate/height/.initial=.8}
\ctikzset{tripoles/xnor gate/port width/.initial=.7}
\ctikzset{tripoles/xnor gate/input height/.initial=.5}
\ctikzset{tripoles/xnor gate/input skip/.initial=.15}
\ctikzset{tripoles/xnor gate/distance/.initial=.1}
\ctikzset{tripoles/xnor gate/aaa/.initial=.6}
\ctikzset{tripoles/xnor gate/bbb/.initial=.4}
\ctikzset{tripoles/xnor gate/ccc/.initial=.5}
\ctikzset{tripoles/xnor gate/ddd/.initial=.0}
\ctikzset{tripoles/xnor gate/circle width/.initial=.15}
\ctikzset{bipoles/buffer/height/.initial=1}
\ctikzset{bipoles/buffer/width/.initial=1}
\ctikzset{bipoles/not gate/width/.initial=1}
\ctikzset{bipoles/not gate/height/.initial=.8}
\ctikzset{bipoles/not gate/circle width/.initial=.15}

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\long\def\pgfcircdeclarelogicgate#1#2{
  \pgfdeclareshape{#1 gate}{
    \savedanchor\northwest{%
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
    }
    \anchor{in 1}{
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/input height}\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
    }
    \anchor{in 2}{
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/input height}\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
      \pgf@y=-\pgf@y
    }
    \anchor{out}{
      \northwest
      \pgf@y=0pt
      \pgf@x=-\pgf@x
    }
    \anchor{center}{
      \northwest
      \pgf@y=0pt
      \pgf@x=0pt
    }
    \backgroundpath{
      \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

      \northwest
      \pgf@circ@res@up=\pgf@y
      \pgf@circ@res@down=-\pgf@y
      \pgf@circ@res@right=-\pgf@x
      \pgf@circ@res@left=\pgf@x

      #2

    }
  }
}

\pgfcircdeclarelogicgate{and}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}{\pgf@circ@res@down}}
  \pgfpathcurveto{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{.5\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{.5\pgf@circ@res@up}}
                 {\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
  \pgfclosepath
  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}
}

\pgfcircdeclarelogicgate{nand}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgfsetlinewidth{2\pgflinewidth}

  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/circle width}\pgf@circ@res@right
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@right

  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
  \pgfpathcurveto{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
                 {\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
  \pgfclosepath

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfsetstrokecolor{black}
  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{nor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}\pgf@circ@res@right
  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/circle width}\pgf@circ@res@right

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{or}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}\pgf@circ@res@right
  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}
}

\pgfcircdeclarelogicgate{xor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}\pgf@circ@res@right
  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/distance}\pgf@circ@res@right+}
  \pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}

  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{xnor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}\pgf@circ@res@right
  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/circle width}\pgf@circ@res@right

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/distance}\pgf@circ@res@right+}
  \pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}

  \pgfusepath{draw}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfusepath{draw}
}

\pgfdeclareshape{not gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfclosepath
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \pgfpathellipse{\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
                   {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
                   {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
    \pgfsetcolor{white}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
  }
}

\pgfdeclareshape{buffer gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{%
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \savedanchor\left{%
    \pgf@y=0pt
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

  }
}

\pgfdeclareshape{tristate buffer gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \savedanchor\left{
    \pgf@y=0pt
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{en}{
    \northwest
    \pgf@x=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \anchor{center}{
    \pgfpointorigin
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0pt}}

    \pgfpathmoveto{\pgfpoint{0pt}{.45\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}

    \pgfusepath{draw}
  }
}

\makeatother

